Kenneth Wilson and lattice QCD

We discuss the physics and computation of lattice QCD, a space-time lattice formulation of quantum chromodynamics, and Kenneth Wilson's seminal role in its development. We start with the fundamental issue of confinement of quarks in the theory of the strong interactions, and discuss how lattice QCD provides a framework for understanding this phenomenon. A conceptual issue with lattice QCD is a conflict of space-time lattice with chiral symmetry of quarks. We discuss how this problem is resolved. Since lattice QCD is a non-linear quantum dynamical system with infinite degrees of freedom, quantities which are analytically calculable are limited. On the other hand, it provides an ideal case of massively parallel numerical computations. We review the long and distinguished history of parallel-architecture supercomputers designed and built for lattice QCD. We discuss algorithmic developments, in particular the difficulties posed by the fermionic nature of quarks, and their resolution. The triad of efforts toward better understanding of physics, better algorithms, and more powerful supercomputers have produced major breakthroughs in our understanding of the strong interactions. We review the salient results of this effort in understanding the hadron spectrum, the Cabibbo-Kobayashi-Maskawa matrix elements and CP violation, and quark-gluon plasma at high temperatures. We conclude with a brief summary and a future perspective.

==> 20150121 for arxiv revised/ukawa-ref.tex <==
% Non-BibTeX users please use
\begin{thebibliography}{}
%
% and use \bibitem to create references. Consult the Instructions
% for authors for reference list style.
%
\bibitem{Wilson1974}
% Format for Journal Reference
K. G. Wilson,  
{\it Confinement of Quarks},  Cornell preprint CLNS-262 (Feb 1974), published in 
Phys. Rev. D10 (1974) 2445. 

\bibitem{Wilson1983}
K. G. Wilson, 
{\it Future Directions in Particle Theory}, 
in Proceedings of the 1983 Lepton Photon Symposium at High Energies, p.812 (Cornell University Press, 1983).

\bibitem{Wilson2005}
K. G. Wilson, 
{\it The Origins of Lattice Gauge Theory}, 
Nucl. Phys. B (Proc. Suppl.) 140 (2005) 3.

\bibitem{CreutzJacobsRebbi1979}
M. Creutz, L. Jacobs, C. Rebbi, 	
{\it Experiments with a Gauge Invariant Ising System}, 
Phys. Rev. Lett. 42 (1979) 1390.  

\bibitem{Wilson1979}
K. G. Wilson, 	
{\it Monte Carlo Calculations for the Lattice Gauge Theory},  
in Proceedings of the 1979 Cargese Summer Institute, NATO Sci. Ser. B59 (1980) 363.

\bibitem{Creutz1979}
M.  Creutz, 
{\it Solving Quantized SU(2) Gauge Theory},  
Brookhaven National Laboratory Print-79-0919 (Sep 1979); 
{\it Monte Carlo Study of Quantized SU(2) Gauge Theory},  
Phys. Rev.  D21 (1980) 2308. 

\bibitem{Weingarten1982}
D. Weingarten, 	
{\it Monte Carlo Evaluation of Hadron Masses in Lattice Gauge Theories with Fermions},  
Phys. Lett. B109 (1982) 57.

\bibitem{HamberParisi1981}
H.  Hamber and G. Parisi, 
{\it Numerical Estimates of Hadronic Masses in a Pure SU(3) Gauge Theory},  
Phys. Rev. Lett. 47 (1981) 1792.  

\bibitem{PDG}
Particle Data Group web page {\tt http://pdg.lbl.gov}

\bibitem{GrossWilczek}
D. J. Gross and F. Wilczek, 
{\it Ultraviolet Behavior of non-Abelian Gauge Theories},
Phys. Rev. Lett.  30 (1974) 1343.

\bibitem{Politzer}
H. D. Politzer, 
{\it Reliable Perturbative Results for Strong Interactions?}, 
Phys. Rev. Lett. 30 (1974) 1346.

\bibitem{Symanzik1969}
K. Symanzik, 
{\it Euclidean quantum field theory}, 
in Local quantum field theory, p. 152,  edited by R. Jost (New York: Academic Press 1969). 

\bibitem{WilsonKogut1973}
K. G. Wilson and J. Kogut, 
{\it The Renormalization Group and the $\epsilon$ Expansion},
Phys. Rep. 12 (1974) 75. 

\bibitem{OsterwalderSchrader1973}
K. Osterwalder, R. Schrader, 
{\it Axioms for Euclidean Green's Functions}, 
Commun. Math. Phys. 31 (1973) 83; 
{\it Axioms for Euclidean Green's Functions II}, 
Commun. Math. Phys. 42 (1975) 281. 

\bibitem{BaliShilling1993}
G. S. Bali, K. Schilling,	
{\it Running Coupling and the Lambda Parameter from SU(3) Lattice Simulations},  
Phys. Rev. D47 (1993) 661.

\bibitem{Bowleretal1986}
K. C. Bowler, A. Hasenfratz, P. Hasenfratz, U. M. Heller, F. Karsch, R. D. Kenway, G. S. Pawley, D. J. Wallace, 
{\it The SU(3) Beta Function at Large Beta}, 
Phys. Lett. B179 (1986) 375.

\bibitem{Guptaetal1988}
R. Gupta, G. W. Kilcup, A. Patel , S. R. Sharpe,
{\it The Beta Function for Pure Gauge SU(3)},  
Phys. Lett. B211 (1988) 132.

\bibitem{Luscheretal1994}
M. L\"uscher, R. Sommer, P. Weisz. U. Wolff,
{\it A Precise Determination of the Running Coupling in the SU(3) Yang-Mills Theory},  
Nucl. Phys. B413 (1994) 481. 

\bibitem{ALpha2005}
ALPHA Collaboration, M. Della Morte, R. Frezzotti, J. Heitger, J. Rolf, R. Sommer, U. Wolff,
{\it Computation of the Strong Coupling in QCD with Two Dynamical Flavours}, 
Nucl. Phys. B713 (2005) 378.

\bibitem{PACS-CS2009a}
PACS-CS Collaboration, S. Aoki, K. I. Ishikawa, N. Ishizuka, T. Izubuchi, D. Kadoh, K. Kanaya, Y. Kuramashi, K. Murano, Y. Namekawa, M. Okawa, Y. Taniguchi, A. Ukawa, N. Ukita, T. Yoshi\'e, 
{\it Precise Determination of the Strong Coupling Constant in $N_f = 2+1$ Lattice QCD with the Schr\"odinger Functional Scheme}, 
JHEP 0910 (2009) 053.

\bibitem{AlphaNf4}
R. Sommer, F. Tekin, U. Wolff,
{\it Running of the SF-coupling with Four Massless Flavours},  
PoS(Lattice 2010) (2010) 241. 

\bibitem{KarstenSmit1981}
L. H. Karsten, J. Smit, 
{\it Lattice Fermions, Species Dubling, Chiral Invariance and the Triangle Anomaly}, 
Nucl. Phys. B183 (1981) 103. 

\bibitem{NielsenNinomiya1981}
H. B. Nielesen and M. Ninomiya, 
{\it Absence of Neutrinos on a Lattice. 1. Proof by Homotopy Theory},  
Nucl. Phys. B185 (1981) 20;  Erratum-ibid. B195 (1982) 541. 

\bibitem{karsten}
L. H. Karsten, 	
{\it Lattice Fermions in Euclidean Space-time}, 
Phys. Lett. B104 (1981) 315.

\bibitem{Wilson1975}
K. G. Wilson, 
{\it Quarks and strings on a lattice}, 
in New Phenomena in Subnuclear Physics, Proceedings of the 14th Course of the International School of Subnuclear Physics, Erice, 1975, edited by A. Zichichi (Plenum, New York, 1977).   

\bibitem{Bochicchioetal1985}
M. Bochicchio, L. Maiani, G. Martinelli, G. C. Rossi, M. Testal,
{\it Chiral Symmetry on the Lattice with Wilson Fermions}, 
Nucl. Phys. B262 (1985) 331.
 
\bibitem{ItohIwasakiOyanagiYoshie1986}
S. Itoh, Y. Iwasaki, Y. Oyanagi, T. Yoshi\'e,
{\it Hadron Spectrum in Quenched  QCD on a $12^3\times 24$ Lattice With Renormalization Group Improved Lattice SU(3) Gauge Action},  
Nucl. Phys. B274 (1986) 33. 

\bibitem{Kawamoto1981}
N. Kawamoto, 	
{\it Towards the Phase Structure of Euclidean Lattice Gauge Theories with Fermions},  
Nucl. Phys. B190 (1981) 617.

\bibitem{Aoki1984}
S. Aoki,
{\it New Phase Structure for Lattice QCD with Wilson Fermions},  
Phys. Rev. D30 (1984) 2653. 

\bibitem{tmQCD2001}
R. Frezzotti, P. Grassi,  S. Sint, P. Weisz,
{\it Lattice QCD with a Chirally Twisted Mass Term}, 
JHEP 0108 (2001) 058.

\bibitem{tmQCD2004}
R. Frezzotti, G. C. Rossi, 
{\it Chirally improving Wilson Fermions - I. O(a) Improvement},
JHEP 08 (2004) 007.

\bibitem{AokiBaer2006}
S. Aoki, O. Baer,
{\it Automatic $O(a)$ Improvement for Twisted Mass QCD in the Presence
of Spontaneous Symmetry Breaking}, 
Phys. Rev. D74 (2006) 034511.

\bibitem{Susskind1977}
L. Susskind, 	
{\it Lattice Fermions},  
Phys. Rev. D16 (1977) 3031.

\bibitem{SharatchandraThusWeisz1981}
H. S. Sharatchandra, H. J. Thus, P. Weisz, 
{\it Susskind Fermions on a Euclidean lattice}, 
Nucl. Phys. B192 (1981) 205. 

\bibitem{KlubergSternetal1981}
H. Kluberg-Stern, A. Morel, O. Napoly, B. Petersson,
{\it Flavors of Lagrangian Susskind Fermions},  
Nucl. Phys. B220 (1983) 447.

\bibitem{Sharpe2006}
S. R. Sharpe, 
{\it Rooted Staggered Fermions: Good, Bad or Ugly?},  
PoS (Lattice 2006) (2006) 022. 

\bibitem{LeeSharpe1999}
W.-J.  Lee, S. R. Sharpe,
{\it Partial Flavor Symmetry Restoration for Chiral Staggered Fermions},  
Phys. Rev. D60 (1999) 114503.  

\bibitem{Wilson1981}
P.  H. Ginsparg and K. G. Wilson, 
{\it A Remnant of Chiral Symmetry on the Lattice}, 
Phys. Rev. D25 (1982) 2649. 
 
 \bibitem{Luescher1998}
M. L\"uscher, 	
{\it Exact Chiral Symmetry on the Lattice and the Ginsparg-Wilson Relation},  
Phys. Lett. B428 (1998) 342. 
 
\bibitem{Kaplan1992}
D. B. Kaplan, 
{\it A Method for Simulating Chiral Fermions on the Lattice},  
Phys. Lett. B288 (1992) 342.

\bibitem{FurmanShamir1995}
V. Furman, Y. Shamir, 
{\it Axial Symmetries in Lattice QCD with Kaplan Fermions}, 
Nucl. Phys. B439 (1995)  54.
 
\bibitem{NarayananNeuberger1995}
R. Narayanan and H. Neuberger 
{\it A Construction of Lattice Chiral Gauge Theories},  
Nucl. Phys. B443 (1995) 305.

\bibitem{Neuberger1998}
H. Neuberger,
{\it Exactly Massless Quarks on the Lattice}, 
Phys. Lett. B417 (1998) 141.

\bibitem{Neuberger1998-2}
H. Neuberger, 
{\it Vector-like Gauge Theories with Almost Massless Fermions on the Lattice}, 
Phys. Rev. D57 (1998) 5417.

\bibitem{Borici1999}
A. Borici, 
{\it Truncated Overlap Fermions}, 
Nucl. Phys. B(Proc. Suppl.) 83 (2000) 771.

\bibitem{HasenfratzNiedermeyer1998}
P. Hasenfratz, V. Laliena, F. Niedermayer,
{\it The Index Theorem in QCD with a Finite Cut-Off }, 
Phys. Lett. B427 (1998) 125. 

\bibitem{RBCUKQCDDomainwall2013}
R. Arthur, T. Blum, P. A. Boyle, N. H. Christ, N. Garron, R. J. Hudspith, T. Izubuchi, C. Jung, C. Kelly, A. T. Lytle, R. D. Mawhinney, D. Murphy, S. Ohta , C. T. Sachrajda, A. Soni, J. Yu, and J. M. Zanotti (RBC and UKQCD Collaborations),
{\it Domain Wall QCD with Near-Physical Pions},  
Phys. Rev. D87 (2013) 094514. 

\bibitem{KEKOverlap2012}
S. Aoki, T.-W. Chiu, G. Cossu, X. Feng, H. Fukaya, S. Hashimoto, T.-H. Hsieh, T. Kaneko, H. Matsufuru, J.  Noaki,
{\it Simulation of Quantum Chromodynamics on the Lattice with Exactly Chiral Lattice Fermions},  
PTEP 2012 (2012) 01A106. 

\bibitem{Hasenfratzetal2005}
A. Hasenfratz, P. Hasenfratz, F. Niedermayer, 
{\it Simulating Full QCD with the Fixed Point Action}, 
Phys. Rev. D72 (2005) 114508.
 
\bibitem{Eichten88}
E. Eichten,
{\it Heavy Quarks on the Lattice},  
Nucl. Phys. Proc. Suppl. 4 (1988) 170. 

\bibitem{LepageThacker88}
G. P. Lepage and B. A. Thacker,	
{\it Effective Lagrangians for Simulating Heavy Quark Systems}, 
Nucl. Phys. Proc. Suppl. 4 (1988) 199.

\bibitem{ElKahdra1997} 
A. X. El-Khadra, A. S. Kronfeld, P. B. Mackenzie
{\it Massive Fermions in Lattice Gauge Theory},  
Phys. Rev. D55 (1997) 3933.

\bibitem{AokiKuramashi2003}
S. Aoki, Y. Kuramashi, S. Tominaga,
{\it Relativistic Heavy Quarks on the Lattice},  
Prog. Theor. Phys. 109 (2003) 383.

\bibitem{ChristLin2007}
N. H. Christ, M. Li, H.-W. Lin,	
{\it Relativistic Heavy Quark Effective Action},  
Phys. Rev. D76 (2007) 074505. 

\bibitem{Metropolis}
N. Metropolis, A. W. Rosenbluth, M. N. Rosenbluth, A. H. Teller, and E. Teller, 
{\it Equation of State Calculations by Fast Computing Machines}, 
Journal of Chemical Physics 21 (1953) 1087.

\bibitem{Wilson1975-2} 
K. G. Wilson, 
{\it The Renormalization Group: Critical Phenomena and the Kondo Problem},  
Rev. Mod. Phys. 47 (1975) 773.  

\bibitem{AndreiLowenstein1981}
N. Andrei, J.H. Lowenstein, 
{\it Scales and Scaling in the Kondo Model}, 
Phys. Rev. Lett. 46 (1981) 356. 

\bibitem{top500}
{\tt http://www.top500.org/lists/2014/11/}

\bibitem{CallawayRahman1982}
D. J. E. Callaway, A. Rahman, 
{\it Microcanonical Ensemble Formulation of Lattice Gauge Theory}, 
Phys. Rev. Lett. 49 (1982) 613.

\bibitem{PolonyiWyld1983}
J. Polonyi, H. W. Wyld, 
{\it Microcanonical Simulation of Fermionic Systems}, 
Phys. Rev. Lett. 51 (1983) 2257.

\bibitem{UkawaFukugita1985}
A. Ukawa. M. Fukugita, 
{\it Langevin Simulation including Dynamical Quark Loops},  
Phys. Rev. Lett. 55 (1985) 1854.

\bibitem{Wilson1985}
G. G. Batrouni, G. R. Katz, A. S. Kronfeld, G. P. Lepage, B.  Svetitsky, K. G. Wilson,
{\it Langevin Simulations of Lattice Field Theories},  
Phys. Rev. D32 (1985) 2736.  

\bibitem{DuaneKennedyPendleton1987}
S. Duane, A. D. Kennedy,  B. J. Pendleton, D. Roweth,  	
{\it Hybrid Monte Carlo},  
Phys. Lett. B195 (1987) 216.

\bibitem{Ukawa2001}
A. Ukawa for CP-PACS and JLQCD Collaborations, 
{\it Computational Cost of Full QCD Simulations experienced by CP-PACS and JLQCD Collaborations},  
Nucl. Phys. B(Proc. Suppl.) 106 (2002) 195.
 
\bibitem{Luescher2005}
M. L\"uscher, 
{\it Schwarz-preconditioned HMC Algorithm for Two-Flavour Lattice QCD},  
Comput. Phys. Commun. 165 (2005) 199.

\bibitem{SextonWeingarten}
J.C. Sexton and D.H. Weingarten, 
{\it Hamiltonian Evolution for the Hybrid Monte Carlo Algorithm}, 
Nucl. Phys. B380 (1992) 665.

\bibitem{PACS-CS2009}
S. Aoki, K.-I. Ishikawa, N. Ishizuka, T. Izubuchi, D. Kadoh, K. Kanaya, Y. Kuramashi, Y. Namekawa, M. Okawa, Y. Taniguchi, A. Ukawa, N. Ukita, and T. Yoshi\'e (PACS-CS Collaboration), 
{\it 2+1 Flavor Lattice QCD toward the Physical Point},  
Phys. Rev. D79 (2009) 034503. 

\bibitem{Hasenbusch}
M.Hasenbusch,
{\it Speeding up the Hybrid Monte Carlo Algorithm for Dynamical Fermions}, 
Phys. Lett.  B519 (2001) 177.

\bibitem{Horvathetal1999}
I. Horvath, A. D. Kennedy, S. Sint, 
{\it A New Exact Method for Dynamical Fermion Computations with Non-local Actions }, 
Nucl. Phys. B(Proc. Suppl.) 73 (1999) 834. 

\bibitem{Luescher2007}
M. L\"uscher, 
{\it Local Coherence and Deflation of the Low Quark Modes in Lattice QCD},  
JHEP 0707 (2007) 081. 

\bibitem{Babichietal2010}
R. Babich, J. Brannick, R. C. Brower, M. A. Clark, T.A. Manteuffel, S. F. McCormick, J. C. Osborn, C. Rebbi, 
{\it Adaptive Multigrid Algorithm for the Lattice Wilson-Dirac Operator},  
Phys. Rev. Lett. 105 (2010) 201602. 

\bibitem{Frommeretal2013}
A. Frommer, K. Kahl, S. Krieg, B. Leder, M. Rottmann, 
{\it Adaptive Aggregation Based Domain Decomposition Multigrid for the Lattice Wilson Dirac Operator},  
e-Print: arXiv:1303.1377 [hep-lat] 

\bibitem{gf11}
F. Butler, H. Chen, J. Sexton, A. Vaccarino, D. Weingarten, 
{\it Hadron Mass Predictions of the Valence Approximation to Lattice QCD},
Phys. Rev. Lett. 70 (1993) 2849.

\bibitem{CP-PACS}
CP-PACS Collaboration: S. Aoki, G. Boyd, R. Burkhalter, S. Ejiri, M. Fukugita, S. Hashimoto, Y. Iwasaki, K. Kanaya, T. Kaneko, Y. Kuramashi, K. Nagai, M. Okawa, H. P. Shanahan, A. Ukawa, T. Yoshi\'e,
{\it Quenched Light Hadron Spectrum},  
Phys. Rev. Lett. 84 (2000) 238. 

\bibitem{CP-PACS2000}
CP-PACS Collaboration: A. Ali Khan, S. Aoki, G. Boyd, R. Burkhalter, S. Ejiri, M. Fukugita, S. Hashimoto, N. Ishizuka, Y. Iwasaki, K. Kanaya, T. Kaneko, Y. Kuramashi, T. Manke, K. Nagai, M. Okawa, H.P. Shanahan, A. Ukawa, T. Yoshi\'e, 
{\it Dynamical Quark Effects on Light Quark Masses}, 
Phys. Rev. Lett. 85 (2000) 4674; Erratum-ibid. 90 (2003) 029902.

\bibitem{BMW2008}
S. Durr, Z. Fodor, J. Frison, C. Hoelbling, R. Hoffmann, S. D. Katz, S. Krieg, T. Kurth, L. Lellouch, T. Lippert, K. K. Szabo, G. Vulvert,
{\it Ab-Initio Determination of Light Hadron Masses},  
Science 322 (2008) 1224. 

\bibitem{Luescher1991}
Martin L\"uscher, 
{\it Two Particle States on a Torus and their Relation to the Scattering Matrix},  
 Nucl. Phys. B354 (1991) 531;  
{\it Signatures of Unstable Particles in Finite Volume},  
Nucl. Phys. B364 (1991) 237. 

\bibitem{DuncanEichtenThacker1996}
A. Duncan, E. Eichten, H. Thacker,
{\it Electromagnetic Splittings and Light Quark Masses in Lattice QCD},  
Phys. Rev. Lett. 76 (1996) 3894.

\bibitem{Blumetal2010}
T. Blum, R. Zhou, T. Doi, M. Hayakawa, T. Izubuchi, S. Uno, N. Yamada,
{\it Electromagnetic Mass Splittings of the Low Lying Hadrons and Quark Masses from 2+1 Flavor Lattice QCD+QED}, 
Phys. Rev. D82 (2010) 094508.

\bibitem{Ishikawaetal2012}
T. Ishikawa, T. Blum, M. Hayakawa, T. Izubuchi,  C. Jung, R. Zhou,
{\it Full QED+QCD Low-Energy Constants through Reweighting},  
Phys. Rev. Lett. 109 (2012) 072002.

\bibitem{PACS-CS2012}
S. Aoki, K.-I. Ishikawa,  N. Ishizuka, K. Kanaya, Y. Kuramashi, Y. Nakamura, Y. Namekawa, M. Okawa, Y. Taniguchi, A. Ukawa, N. Ukita, T. Yoshi\'e (PACS-CS Collaboration),
{1+1+1 flavor QCD + QED Simulation at the Physical Point},  
Phys. Rev. D86 (2012) 034507. 

\bibitem{BMW2014}
S. Borsanyi, S. Durr, Z. Fodor, C. Hoelbling, S. D. Katz, S. Krieg, L. Lellouch, T. Lippert, A. Portelli,
K. K. Szabo,
{\it Ab initio Calculation of the Neutron-Proton Mass Difference},  
arXiv:1406.4088 (2014).

\bibitem{Ishizuka2007} 
S. Aoki, M. Fukugita, K-I. Ishikawa, N. Ishizuka, K. Kanaya, Y. Kuramashi, Y. Namekawa, M. Okawa, K. Sasaki, A. Ukawa, and T. Yoshi\'e, 
{\it Lattice QCD Calculation of the $\rho$ Meson Decay Width}, 
Phys. Rev. D 76 (2007) 094506;
{\it $\rho$ Meson Decay in $2+1$ Flavor Lattice QCD}, 
Phys. Rev. D84 (2011) 094505.

\bibitem{MILC09}
A. Bazavov, C. Bernard, C. DeTar, X. Du, W. Freeman, S. Gottlieb, U. M. Heller, J. E. Hetrick, J. Laiho, L. Levkova, M. B. Oktay, J. Osborn, R. Sugar, D. Toussaint, R. S. Van de Water (The MILC Collaboration), 
{\it MILC Results for Light Pseudo Scalars}, 
PoS (CD09) (2009) 007.

\bibitem{BMW2010}
S. Durr, Z. Fodor, C. Hoelbling, S. Katz, S. Krieg et al., 
{\it Lattice QCD at the Physical Point: Light Quark Masses}, 
Phys. Lett. B701 (2011) 265.

\bibitem{PDG1998}
Particle Data Group Collaboration (C. Caso {\it et al.}), 	
{\it Review of Particle Physics}, 
Eur. Phys. J. C3 (1998) 1. 

\bibitem{PDG2012}
Particle Data Group Collaboration (J. Beringer {\it et al.}), 	
{\it Review of Particle Physics}, 
Phys. Rev. D86 (2012) 010001. 

\bibitem{PDG2013revision}
"Quantum Chromodyamics" section in {\tt http://pdg.lbl.gov/2013/reviews/}.

\bibitem{HPQCD2010}
C. McNeile, C. T. H. Davies, E. Follana, K. Hornbostel, G. P. Lepage,
{\it High-Precision c and b Masses and QCD Coupling from Current-Current Correlators in Lattice and Continuum QCD}, 
Phys. Rev. D82 (2010) 034512.

\bibitem{Bazavov2012}
A. Bazavov, N. Brambilla, X. Garcia i Tormo, P. Petreczky, J. Soto, A. Vairo, 
{\it Determination of $\alpha_s$ from the QCD Static Energy}, 
Phys. Rev. D86 (2012) 114031.

\bibitem{UTfitter}
{\tt http://www.utfit.org/UTfit/}

\bibitem{CKMfitter}
{\tt http://http://ckmfitter.in2p3.fr}
 
\bibitem{HFAG}
{\tt http://www.slac.stanford.edu/xorg/hfag/}

\bibitem{FLAG2014}
FLAG Working Group, S. Aoki, Y. Aoki, C. Bernard, T. Blum, G. Colangelo, M. Della Morte, S. Durr,
A. X. El-Khadra, H. Fukaya, R. Horsley, A. Juttner, T. Kaneko, J. Laiho,
L. Lellouch, H. Leutwyler, V. Lubicz, E. Lunghi, S. Necco, T. Onogi, C. Pena, C. T. Sachrajda, S. R. Sharpe, S. Simula, R. Sommer, R. S. Van de Water, A. Vladikas, U. Wenger, H. Wittig,
{\it Review of Lattice Results concerning Low Energy Particle Physics}, 
ArXive:1310.8555 ( August 2014).

\bibitem{FNAL2012}
A. Bazavov, C. Bernard, C. M. Bouchard, C. DeTar, M. Di Pierro, A. X. El-Khadra, R. T. Evans, E. D. Freeland, E. Gamiz, S. Gottlieb, U. M. Heller, J. E. Hetrick, R. Jain, A. S. Kronfeld, J. Laiho, L. Levkova, P. B. Mackenzie, E. T. Neil, M. B. Oktay, J. N. Simone, R. Sugar, D. Toussaint, R. S. Van de Water,
{\it Neutral B-meson Mixing from Three-Flavor Lattice QCD: Determination of the SU(3)-Breaking Ratio $\xi$}, 
Phys. Rev. D86 (2012) 034503.

\bibitem{HPQCD2006}
E. Gulez, A. Gray, M. Wingate, C. T. H. Davies, G. P. Lepage, J. Shigemitsu, 
{\it B Meson Semileptonic Form Factors from Unquenched Lattice QCD}, 
Phys. Rev. D73 (2006) 074502.

\bibitem{FNAL2008}
J. A. Bailey, C. Bernard, C. DeTar, M. Di Pierro, A. X. El-Khadra, R. T. Evans, E. D. Freeland, E. Gamiz, S. Gottlieb, U. M. Heller, J. E. Hetrick, A. S. Kronfeld, J. Laiho, L. Levkova, P. B. Mackenzie, M. Okamoto, J. N. Simone, R. Sugar, D. Toussaint, R. S. Van de Water, 
{\it The $B\to\pi\ell\nu$ Semi-Leptonic Form Factor from Three-Flavor Lattice QCD: A Model-Independent Determination of $\vert V_{ub}\vert$}, 
Phys. Rev. D79 (2009) 054507. 

\bibitem{FNAL2014}
J. A. Bailey, A. Bazavov, C. Bernard, C. M. Bouchard, C. DeTar, D. Du, A. X. El-Khadra, J. Foley, E. D. Freeland, E. G\'amiz, S. Gottlieb, U. M. Heller, A. S. Kronfeld, J. Laiho, L. Levkova, P. B. Mackenzie, E. T. Neil, S.-W. Qiu, J. Simone, R. Sugar, D. Toussaint, R. S. Van de Water, R. Zhou, 
{\it Update of $\vert V_{cb} \vert$ from the $\overline{B}\to D^{*}\ell\overline{\nu}$ Form Factor at Zero Recoil with Three-Flavor Lattice QCD}, 
Phys. Rev. D89 (2014) 114504.

\bibitem{NA48}
V. Fanti {\it et al}, 
{\it A New Measurement of Direct CP Violation in Two Pion Decays of the Neutral Kaon}, 
Phys. Lett. B465 (1999) 335.

\bibitem{KTeV}
A. Arabi-Harati {\it et al}, 
{\it Measurements of Direct CP Violation, CPT Symmetry, and Other Parameters in the Neutral Kaon System}, 
Phys. Rev. D67 (2003) 012005.

\bibitem{Buras}
G. Buchalla, A. J. Buras, M. K. Harlander,
{\it The Anatomy of $\epsilon'/\epsilon$ in the Standard Model }, 
Nucl. Phys. B337 (1990) 313;
G. Buchalla, A. J. Buras, M. E. Lautenbacher,
{\it Weak Decays beyond Leading Logarithms},  
Rev. Mod. Phys. 68 (1996) 1125.  

\bibitem{Doninietal1999}
A. Donini, V. Gimenez, G. Martinelli, M. Talevi, A. Vladikas, 
{\it Non-Perturbative Renormalization of Lattice Four-Fermion Operators without
Power Subtractions}, 
Eur. Phys. J. C10 (1999) 121.

\bibitem{Ishizuka2013}
N. Ishizuka, K. I. Ishikawa, A. Ukawa, T. Yoshi\'e,
{\it Calculation of $K\to\pi\pi$ Decay Amplitudes with Improved Wilson Fermion},  
arXiv:1311.0958(2013).
  
\bibitem{LelloucheLuscher}
L. Lellouch, M. L\"uscher,
{\it Weak Transition Matrix Elements from Finite Volume Correlation Functions},  
Commun. Math. Phys. 219 (2001) 31.

\bibitem{RBRC2012}
T. Blum, P. A. Boyle, N. H. Christ, N. Garron, E. Goode, T. Izubuchi, C. Jung, C. Kelly, C. Lehner, M. Lightman,
{\it The $K\to(\pi\pi)_{I=2}$ Decay Amplitude from Lattice QCD},  
Phys. Rev. Lett. 108 (2012) 141601; Phys. Rev. D86 (2012) 074513. 
 
\bibitem{Columbia1990}
F. R. Brown, F. P. Butler, H. Chen, N. H. Christ,  Z.-H. Dong, W. Schaffer, L. I. Unger, A. Vaccarino, 	
{\it On the Existence of a Phase Transition for QCD with Three Light Quarks}, 
Phys. Rev. Lett. 65 (1990) 2491.

\bibitem{Kanaya2010}
K. Kanaya,
{\it Finite Temperature QCD on the Lattice -- Status 2010},  
PoS (Lattice 2010) (2010) 012. 
 
\bibitem{Polyakov}
A. M. Polyakov,
{\it Thermal Properties of Gauge Fields and Quark Liberation}, 
Phys. Lett. 72B (1978) 477.

\bibitem{Susskind}
L. Susskind, 
{\it Hot Quark Soup}, 
Phys. Rev. D20 (1979)  2610.

\bibitem{YaffeSvetitsky}
L. G. Yaffe, B. Svetitsky,
{\it First Order Phase Transition in the SU(3) Gauge Theory at Finite Temperature},  
Phys. Rev. D26 (1982) 963. 

\bibitem{BanksUkawa} 
T. Banks, A. Ukawa,
{\it Deconfining and Chiral Phase Transitions in Quantum Chromodynamics at Finite Temperature},  
Nucl. Phys. B225 (1983) 145. 

\bibitem{PisarskiWilczek}
R. D. Pisarski, F. Wilczek,
{\it Remarks on the Chiral Phase Transition in Chromodynamics},  
Phys. Rev. D29 (1984) 338.

\bibitem{GavinGokschPisarski}
S. Gavin, A. Gocksch, R.  D. Pisarski,
{\it QCD and the Chiral Critical Point }, 
Phys. Rev. D49 (1994) 3079.

\bibitem{Rjagopal1995}
K. Rajagopal, 
{\it The Chiral Phase Transition in QCD: Critical Phenomena and Long Wavelength Pion Oscillations},  
Quark-gluon plasma vol.2 (1995) (arXiv: hep-ph/9504310).

\bibitem{FSS}
For example, see, M. N. Barber, 
{\it Finite Size Scaling}, 
Phase Transitions and Critical Phenomena Vol. 8 (1973), edited by C. Domb and J. Lewobitz (Academic Press).

\bibitem{FukugitaOkawaUkawa}
M. Fukugita, M. Okawa, A. Ukawa,  
{\it Order of the Deconfining Phase Transition in SU(3) Lattice Gauge Theory},  
Phys. Rev. Lett. 63 (1989) 1768;
{\it Finite Size Scaling Study of the Deconfining Phase Transition in Pure SU(3) Lattice Gauge Theory},  
Nucl. Phys. B337 (1990) 181.  

\bibitem{Kayaetal1999}
JLQCD Collaboration: S. Aoki, M. Fukugita, S. Hashimoto, K-I. Ishikawa, N. Ishizuka, Y. Iwasaki, K. Kanaya, T. Kaneda, S. Kaya , Y. Kuramashi, M. Okawa, T. Onogi,
S. Tominaga, N. Tsutsui, A. Ukawa, N. Yamada, T. Yoshi\'e, 
{\it Phase Structure of Lattice QCD at Finite Temperature for 2+1 Flavors of Kogut-Susskind Quarks},  
Nucl. Phys. B (Proc.Suppl.) 73 (1999) 459.

\bibitem{Karschetal2001}
F. Karsch, E. Laermann, C. Schmidt, 
{\it The Chiral Critical Point in Three-Flavor QCD},  
Phys. Lett. B520 (2001) 41.
 
\bibitem{Dingetal2011}
H.-T. Ding, A. Bazavov, P. Hegde, F. Karsch, S. Mukherjee, P. Petreczky,
{\it Exploring Phase Diagram of $N_f=3$ QCD at $\mu=0$ with HISQ Fermions},  
PoS (Lattice 2011) (2011) 191. 

\bibitem{JLQCDNf2Thermo}
S. Aoki, M. Fukugita, S. Hashimoto, N. Ishizuka, Y. Iwasaki, K. Kanaya, Y. Kuramashi, H. Mino, M. Okawa, A. Ukawa, and T. Yoshi\'e (JLQCD Collaboration), 
{\it Scaling Study of the Two Flavor Chiral Phase Transition with the Kogut-Susskind Quark Action in Lattice QCD},  
Phys. Rev. D57 (1998) 3910.

\bibitem{CP-PACSThermoNf2001}
A. Ali Khan, S. Aoki, R. Burkhalter, S. Ejiri, M. Fukugita, S. Hashimoto, N. Ishizuka, Y. Iwasaki, K. Kanaya, T. Kaneko, Y. Kuramashi, T. Manke, K. Nagai, M. Okamoto, M. Okawa, A. Ukawa, and T. Yoshi\'e (CP-PACS Collaboration)), 
{\it Phase Structure and Critical Temperature of Two Flavor QCD with Renormalization Group Improved Gauge Action and Clover improved Wilson Quark Action},  
Phys. Rev. D63 (2001) 034502. 

\bibitem{Bonatietal2009}
C. Bonati, G. Cossu, M. D'Elia, A. Di Giacomo, C. Pica, 
{\it The Order of the QCD Transition with Two Light Flavors},  
Nucl. Phys. A820 (2009) 243C. 

\bibitem{AokiFukayaTaniguchi}
S. Aoki, H. Fukaya, Y. Taniguchi, 
{\it Chiral Symmetry Restoration, the Eigenvalue Density of the Dirac Operator, and the Axial U(1) Anomaly at Finite Temperature}, 
Phys. Rev. D 86 (2012) 114512. 

\bibitem{Bernardetal1997}
C. Bernard, T. Blum, C. DeTar, S. Gottlieb, U. M. Heller, J. E. Hetrick, K. Rummukainen, R. Sugar, D. Toussaint, M. Wingate, 
{\it Which Chiral Symmetry is Restored in High Temperature Quantum Chromodynamics?}, 
Phys. Rev. Lett. 78 (1997) 598. 

\bibitem{Columbia1999}
S. Chandrasekharan, D. Chen, N. Christ, W. J. Lee, R. Mawhinney, P. Vranas,
{\it Anomalous Chiral Symmetry Breaking above the QCD Phase Transition}, 
Phys. Rev. Lett. 82 (1999) 2463. 

\bibitem{WB2006}
Y. Aoki, G. Endrodi, Z. Fodor, S. D. Katz, K. K. Szabo,
{\it The Order of the Quantum Chromodynamics Transition predicted by the Standard Model of Particle Physics},  
Nature 443 (2006) 675. 

\bibitem{WBTc2010}
Y. Aoki, Z. Fodor, S.D. Katz, K.K. Szabo, 
{\it The QCD Transition Temperature: Results with Physical Masses in the Continuum Limit}, 
Phys. Lett. B643 (2006) 46; 
Wuppertal-Budapest Collaboration, S. Borsanyi, Z. Fodor, C. Hoelbling, S. D.  Katz, S. Krieg, C. Ratti, K.  K. Szabo, 
{\it  Is There still any $T_c$ Mystery in Lattice QCD? Results with Physical Masses in the Continuum Limit III},  
JHEP 1009 (2010) 073. 

\bibitem{WBEoS2014}
S. Borsanyi, Z. Fodor, C. Hoelbling, S. D. Katz, S. Krieg. K. K. Szabo,
{\it Full Result for the QCD Equation of State with 2+1 Flavors},  
Phys. Lett. B730 (2014) 99. 

\bibitem{HotQCD2012}
A. Bazavov, T. Bhattacharya, M. Cheng, C. DeTar, H.-T. Ding, S. Gottlieb, R. Gupta, P. Hegde, U. M. Heller, F. Karsch, E. Laermann, L. Levkova, S. Mukherjee, P. Petreczky, C. Schmidt, R. A. Soltz, W. Soeldner, R. Sugar, D. Toussaint, W. Unger, and P. Vranas (HotQCD Collaboration),
{\it Chiral and Deconfinement Aspects of the QCD Transition}, 
Phys. Rev. D 85 (2012) 054503.

\bibitem{HotQCD2014}	
HotQCD Collaboration, A. Bazavov, T. Bhattacharya, C. DeTar, H.-T. Ding, S. Gottlieb, R. Gupta, P. Hegde, U. M. Heller, F. Karsch, E. Laermann, L. Levkova, S. Mukherjee, P. Petreczky, C. Schmidt, C. Schroeder, R. A. Soltz, W. Soeldner, R. Sugar, M. Wagner, P. Vranas, 
{\it The Equation of State in 2+1-Flavor QCD},  
e-Print: arXiv:1407.6387 (2014) 

\bibitem{PHENIX2005} PHENIX Collaboration, S. S. Adler {\it et al.}, 
{\it Systematic Studies of the Centrality and $\sqrt{s_{NN}}$ Dependence of the $dE_T /d\eta$ 
 and $dN_{ch}/d\eta$ in Heavy Ion Collisions at Mid-rapidity}, 
Phys. Rev. C71 (2005) 034908.

\bibitem{CMS2012} CMS Collaboration, S. Chatrchyan {\it et al.}, 
{\it Measurement of the Pseudorapidity and Centrality Dependence of the Transverse Energy Density in Pb--Pb Collisions at $\sqrt{s_{NN}}=2.76$~TeV}, 
Phys. Rev. Lett. 109 (2012) 152303. 

\bibitem{PHENIX2010} PHENIX Collaboration, 
{\it Enhanced Production of Direct Photons in Au+Au Collisions at $\sqrt{s_{NN}}=200$~GeV and Implications for the Initial Temperature}, 
Phys. Rev. Lett. 104 (2010) 132301. 

\bibitem{ALICE2012} 
M. Wilde for ALICE Collaboration, 
{\it Measurement of Direct Photons in pp and Pb-Pb Collisions with ALICE}, 
arXiv.1210.5958 (2012)

\bibitem{Andronic2009}
A. Andronica, P. Braun-Munzinger, J. Stachel,
{\it Thermal Hadron Production in Relativistic Nuclear Collisions: The Hadron Mass Spectrum, the Horn, and the QCD Phase Transition}, 
Phys. Lett. B673 (2009) 142.

\bibitem{Kovtunetal2005}
P. Kovtun, D. T. Son, A.  O. Starinets,
{\it Viscosity in Strongly Interacting Quantum Field Theories from Black Hole Physics}, 
Phys. Rev. Lett. 94 (2005) 111601.

\bibitem{NakamuraSakai2006}
A. Nakamura, S. Sakai,
{\it Lattice Study of Gluon Viscosities: A Step towards RHIC Physics},  
Acta Phys. Polon. B37 (2006) 3371. 

\bibitem{Meyer2007} 
H. B. Meyer, 
{\it A Calculation of the Shear Viscosity in SU(3) Gluodynamics},  
Phys. Rev. D76 (2007) 101701(R). 

\bibitem{Stephanovetal1999}
M. Stephanov, K. Rajagopal, E. Shyuriak, 
{\it Event-by-Event Fluctuations in Heavy Ion Collisions and the QCD Critical Point}, 
Phys. Rev. D60 (1999) 114028.

\bibitem{EjiriKarschRedlich2006}
S. Ejiri, F. Karsch, K. Redlich,
{\it Hadronic Fluctuations at the QCD Phase Transition}, 
Phys. Lett. B 633 (2006) 275.

\bibitem{Karsch2012}
F. Karsch,
{\it Determination of Freeze-out Conditions from Lattice QCD Calculations}, 
Centr. Eur. J. phys. 10 (2102) 1234.

\bibitem{Bazabovetal2012}
A. Bazavov, H.-T. Ding, P. Hegde, O. Kaczmarek, F. Karsch,E. Laermann,  S. Mukherjee, P. Petreczky, C. Schmidt, D. Smith,  W. Soeldner, M. Wagner,
{\it Freeze-Out Conditions in Heavy Ion Collisions from QCD Thermodynamics}, 
Phys. Rev. Lett. 109 (2012) 192302.

\bibitem{Borsanyietal2014}
S. Borsanyi, Z. Fodor, S. D. Katz, S. Krieg, C. Ratti, K. K. Szabo,
{\it Freeze-Out Parameters from Electric Charge and Baryon Number Fluctuations: Is There Consistency?}, 
Phys. Rev. Lett. 113 (2014) 052301.

\bibitem{FodorKatz2001}
Z. Fodor, S. D. Katz, 	
{\it A New Method to Study Lattice QCD at Finite Temperature and Chemical Potential},  
Phys. Lett. B534 (2002) 87;
{\it Lattice Determination of the Critical Point of QCD at Finite T and $\mu$},  
JHEP 0203 (2002) 014.  

\bibitem{RobergeWeiss1986}
A.  Roberge, N. Weiss, 
{\it Gauge Theories with Imaginary Chemical Potential and the Phases of QCD},
Nucl. Phys. B275 (1986) 734.

\bibitem{ForcrandPhilipsen2002}
P. de Forcrand, O. Philipsen, 
{\it The QCD Phase Diagram for Small Densities from Imaginary Chemical Potential}, 
Nucl. Phys. B642 (2002) 290.

\bibitem{Alltonetal2003}
C. R. Allton, S. Ejiri, S. J. Hands, O. Kaczmarek, F. Karsch, E. Laermann, C. Schmidt,
{\it The Equation of State for Two Flavor QCD at Non-zero Chemical Potential},  
Phys. Rev. D68 (2003) 014507.

\bibitem{Ejirietal2012}
S. Ejiri, K. Kanaya, T.  Umeda, 
{\it Ab Initio Study of the Thermodynamics of Quantum Chromodynamics on the Lattice at Zero
and Finite Densities}, 
PTEP 2012 (2012) 01A104.

\bibitem{Lietal}
A.  Li, A. Alexandru, K.-F. Liu,  X. Meng,
{\it Finite Density Phase Transition of QCD with $N_f=4$ and $N_f=2$ using Canonical Ensemble Method},  
Phys. Rev. D82 (2010) 054502;
A. Li, A. Alexandrou, K.-F. Liu, 
{\it Critical Point of Nf=3 QCD from Lattice Simulations in the Canonical Ensemble},  
Phys. Rev. D84 (2011) 071503.  

\bibitem{Aartsetal}
G. Aarts, I.-O. Stamatescu, 	
{\it Stochastic Quantization at Finite Chemical Potential},  
JHEP 0809 (2008) 018;
G. Aarts, E. Seiler, I.-O. Stamatescu,
{\it The Complex Langevin Method: When can It be trusted?}, 
Phys. Rev. D81 (2010) 054508.  

\bibitem{Sexty2013}
D. Sexty, 
{\it Simulating full QCD at Non-zero Density using the Complex Langevin Equation},  
Phys. Lett. B729 (2014) 108. 

\bibitem{Mackenzie1985}
P. B. Mackenzie and H. B. Thacker, 
{\it Evidence Against a Stable Dibaryon from Lattice QCD}, 
Phys. Rev. Lett. 55 (1985) 2539.

\bibitem{Iwasaki1988}
Y. Iwasaki,T. Yoshi\'e, Y. Tsuboi,
{\it The H Dibaryon in Lattice QCD},
Phys. Rev. Lett. 60 (1988) 1371.

\bibitem{Fukugitaetal1994}
M. Fukugita, Y. Kuramashi, H. Mino, M. Okawa, A. Ukawa, 
{\it An Exploratory Study of Nucleon-Nucleon Scattering Lengths in Lattice QCD},
Phys. Rev. Lett. 73 (1994) 2176; 
M. Fukugita, Y. Kuramashi, M. Okawa, H. Mino, A. Ukawa, 
{\it Hadron Scattering Lengths in Lattice QCD}, 
Phys. Rev. D52 (1995) 3003.

\bibitem{Ishiietal2007}
N. Ishii, S. Aoki, T. Hatsuda,
{\it The Nuclear Force from Lattice QCD},  
Phys. Rev. Lett. 99 (2007) 022001. 

\bibitem{Yamazakietal2009}
T. Yamazaki, Y. Kuramashi, and A. Ukawa  (PACS-CS Collaboration),	
{\it Helium Nuclei in Quenched Lattice QCD}, 
Phys. Rev. D81 (2010) 111504.
 
 \bibitem{Lax1982}
 P. D. Lax, chairman, 
 {\it report of the panel on Large Scale Computing in Science and Engineering}, 
 1982  (scanned pdf file is found at {\tt http://www.pnl.gov/scales/docs/lax\_report1982.pdf}).
 
\end{thebibliography}

